Topology of the space of locally convex curves on the 3-sphere

A (positive) locally convex curve in the 2-sphere is a curve with positive geodesic curvature (i.e., which always turns left). In the 3-sphere, it is a curve with positive torsion. In this work we discussed the topology of spaces of such curves with prescribed initial and final jets. The case of the 2-sphere is understood (Saldanha-2013); the case of n=3 is not yet thoroughly clarified. In order to obtain partial information about the homotopy type of such spaces in the case n=3, we represented a positive locally convex curve as a pair of curves on the 2-sphere with some restrictions.

==> Makefile <==
##############################################################################
#
# Makefile for LaTeX files
# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile
# First modification by Matti Airas <Matti.Airas@hut.fi>
# Second modification by Thomas Lewiner <lewiner@gmail.com>
# Third modification by Americo Barbosa da Cunha Jr <americo.cunhajr@gmail.com>
# last update: Jan 4, 2010
#
##############################################################################


######################### Programs ################################

#LATEX	  = pdflatex --shell-escape -interaction=nonstopmode
LATEX	  = latex -src-specials -interaction=nonstopmode
BIBTEX	  = bibtex
MAKEINDEX = makeindex
XDVI	  = xdvi -gamma 4
DVIPS	  = dvips
DVIPDF    = dvipdfmx
L2H	  = latex2html -split 0
TTH	  = tth #-a -e2
GH	  = gv
XPDF	  = xpdf
RM        = rm -Rf


########################## Sources ################################

# BEGIN DEPENDENCIES

SRC       := example.tex
CLASSES   := puc-rio_thesis.cls
STYLES    := atbeginend.sty chngpage.sty nomencl.sty
INPUTS    := *.tex
BIBFILE   := bibliography.bib
BIBSTYLES := puc-rio_num_us.bst puc-rio_bib_us.bst
INPUTENCS := noaccent.def
EPSPICS   := puc_logo.eps

# END DEPENDENCIES


DVI	 = $(SRC:%.tex=%.dvi)
PSF	 = $(SRC:%.tex=%.ps)
PDF	 = $(SRC:%.tex=%.pdf)
HTM	 = $(SRC:%.tex=%_htm)
HTML	 = $(SRC:%.tex=%.html)


####################### Dependencies ##############################


ifeq ($(MAKECMDGOALS),depend)

SRC     := $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)

CLASSES := $(shell perl -ne '($$_)=/^[^%]*\\documentclass[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.cls "}' $(SRC))
CLASSES := $(sort $(foreach class,$(CLASSES), $(shell if [ -f $(class) ] ; then echo $(class) ; else echo class $(class) not in folder >&2 ; fi ;) ) )

STYLES  := $(shell perl -ne '($$_)=/^[^%]*\\[useRqir]+[Pp]ackage[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.sty "}' $(SRC) $(CLASSES))
STYLES  := $(sort $(foreach style,$(STYLES), $(shell if [ -f $(style) ] ; then echo $(style) ; else echo style $(style) not in folder >&2 ; fi ;) ) )

BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
BIBFILE := $(sort $(foreach bibfile,$(BIBFILE), $(shell if [ -f $(bibfile) ] ; then echo $(bibfile) ; else echo bibfile $(bibfile) not in folder >&2 ; fi ;) ) )

BIBSTYLES := $(shell perl -ne '($$_)=/^[^%]*\\bibliographystyle[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bst "}' $(SRC) $(INPUTS) $(CLASSES) $(STYLES))
BIBSTYLES := $(sort $(foreach bibstyle,$(BIBSTYLES), $(shell if [ -f $(bibstyle) ] ; then echo $(bibstyle) ; else echo bibstyle $(bibstyle) not in folder >&2 ; fi ;) ) )

INPUTS  := $(shell perl -ne '($$_)=/^[^%]*\\input\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.tex "}' $(SRC) $(CLASSES) $(STYLES) $(BIBSTYLES) )
INPUTS  := $(sort $(foreach input,$(INPUTS), $(shell if [ -f $(input) ] ; then echo $(input) ; else echo input file $(input) not in folder >&2 ; fi ;) ) )

INPUTENCS := $(shell perl -ne '($$_)=/^[^%]*\\inputencoding\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.def "}' $(SRC) $(CLASSES) $(STYLES) $(BIBSTYLES) )
INPUTENCS := $(sort $(foreach inputenc,$(INPUTENCS), $(shell if [ -f $(inputenc) ] ; then echo $(inputenc) ; else echo inputenc $(inputenc) not in folder >&2 ; fi ;) ) )

EPSPICS := \
  $(shell perl -ne '($$_)=/^[^%]*\\includegraphics[^{}]*\{([^@\#]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) $(CLASSES) $(STYLES) $(BIBSTYLES) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\[tvsingleubo]+image[{[].*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "figs/$$b "}' $(SRC) $(INPUTS) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\watermark[^{}]*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\logouni[^{}]*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) )
EPSPICS := $(sort $(foreach fig,$(EPSPICS), $(shell if [ -f $(fig) ] ; then echo $(fig) ; else if [ -f $(fig).eps ] ;  then echo $(fig).eps ; else if [ -f $(fig).ps ] ;  then echo $(fig).ps ; else if [ -f $(fig).png ] ;  then echo $(fig).png ; else echo figure $(fig) not in folder >&2 ; fi ; fi ; fi ; fi ;) ) )

endif


######################### Messages ################################

RERUN     = "(!|(There were undefined references|Rerun to get (cross-references|the bars) right))"
RERUNBIB  = "No file.*\.bbl|Citation.*undefined"
MAKEIDX   = "^[^%]*\\makeindex"
MPRINT    = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
OUTDATED  = echo "EPS-file is out-of-date!" && false


########################## Macros #################################

define run-latex
	if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi && \
	if test -r $(<:%.tex=%.idx); then cp $(<:%.tex=%.idx) $(<:%.tex=%.idx.bak); fi && \
	$(LATEX) $< > /dev/null ; true
endef


define rerun-latex
	if cmp -s $(<:%.dvi=%.tex) $(<:%.dvi=%.tex.bak) ; \
	  then rm $(<:%.dvi=%.tex.bak) ; \
	  else \
	    touch -r $(<:%.dvi=%.tex) $(<:%.dvi=%.tex.bak) ; \
	    mv $(<:%.dvi=%.tex.bak) $(<:%.dvi=%.tex) ; \
	    $(run-latex) ; \
	    touch -r $(<:%.dvi=%.tex) $< ; \
	fi
endef


define run-complete
	$(run-latex)
    $(MAKEINDEX) $(SRC:%.tex=%.nlo) -s nomencl.ist -o $(SRC:%.tex=%.nls)
	( egrep -q $(MAKEIDX) $< > /dev/null && \
    ! (cmp -s $(<:%.tex=%.idx) $(<:%.tex=%.idx.bak)) ) && ( \
    $(MAKEINDEX) $(<:%.tex=%) 2>&1 | egrep -i "(lines|error)" ; $(run-latex) ) ; true
	( for file in $(BIBFILE) ; do if [ $file -nt $(<:%.tex=%.bbl) ] ; then \
    $(BIBTEX) $(<:%.tex=%) | egrep -i "(Database|error)" ; $(run-latex) ; break ; fi; done ; ) ; true
  ( egrep -q $(RERUNBIB) $(<:%.tex=%.log) > /dev/null && \
    $(BIBTEX) $(<:%.tex=%) | egrep -i "(Database|error)" ; $(run-latex) ) ; true
	egrep -q $(RERUN) $(<:%.tex=%.log) > /dev/null && $(run-latex) ; true
	egrep -q $(RERUN) $(<:%.tex=%.log) > /dev/null && $(run-latex) ; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak) ; then true ; else $(run-latex) ; fi
	$(RM) $(<:%.tex=%.toc.bak) $(<:%.tex=%.idx.bak)
endef


define show-warnings
	if test -e $(<:%.tex=%.blg) ; then \
    egrep -B1 -A3 -i "line " $(<:%.tex=%.blg) ; \
	  egrep -i "Warning-" $(<:%.tex=%.blg) ; \
  fi ; true
	if test -e $(<:%.tex=%.log) ; then \
    egrep -i "Overful" $(<:%.tex=%.log) ; \
    egrep -i "Warning" $(<:%.tex=%.log) ; \
    egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; \
    egrep -A3 -i "^!" $(<:%.tex=%.log) ; \
  fi ; true
endef

define show-stats
	if test -e $(<:%.tex=%.ilg) ; then \
    echo -n "Index  : " ; egrep -i "Generating" $(<:%.tex=%.ilg) ; \
  fi ; true
	if test -e $(<:%.tex=%.blg) ; then \
    echo -n "BibTeX : " ; egrep -i "entries" $(<:%.tex=%.blg) ; \
  fi ; true
	if test -e $(<:%.tex=%.log) ; then \
	  echo -n "LaTeX  : " ; egrep -i "written" $(<:%.tex=%.log) ; \
  fi ; true
	if test -e $(<:%.tex=%.aux) ; then \
    echo -n "         " ; \
    echo -n $(shell egrep -c "contentsline {chapter}" $(<:%.tex=%.aux)) ; echo -n " chapters, " ; \
    echo -n $(shell egrep -c "contentsline {section}" $(<:%.tex=%.aux)) ; echo -n " sections and, " ; \
    echo -n $(shell egrep -c "contentsline {subsection}" $(<:%.tex=%.aux)) ; echo " subsections." ; \
  fi ; true
endef


####################### File Targets ##############################

dvi	 : $(DVI)

ps	 : $(PSF) 

pdf	 : $(PDF) 

htm	 : $(HTM)

html : $(HTML)

DIRNAME = $(notdir ${PWD})
TARNAME = ../$(shell echo $(DIRNAME) | tr [:upper:] [:lower:]).tgz
tar  : $(TARNAME)


###################### default targets ############################

all 	  :
	make depend
	@for i in $(DVI) ; do if egrep -q -i $(RERUN) $${i/.dvi/.log} ; then $(RM) $$i ; fi ; done ; true
	make dvi

everything :
	make depend
	@for i in $(DVI) ; do if egrep -q -i $(RERUN) $${i/.dvi/.log} ; then $(RM) $$i ; fi ; done ; true
	make dvi
	@for i in $(PSF) $(PDF) $(HTML) $(HTM) ; do if test -r $$i ; then make $$i ; fi ; done ; true
	make tar
	make cvs

.PHONY	: all everything depend warns stats show-depend clean dvi ps pdf htm html show showps showpdf tar cvs


##################### Programs Targets ############################

show	: $(DVI)
	@for i in $(DVI) ; do $(XDVI) $$i ; done

showps	: $(PSF)
	@for i in $(PSF) ; do $(GH) $$i ; done

showpdf	: $(PDF)
	@for i in $(PDF) ; do $(XPDF) $$i ; done

clean	:
	$(RM) .\#* *~ $(DVI) $(PSF) $(PDF) $(HTM) $(HTML) \
  $(DVI:%.dvi=%.aux) $(DVI:%.dvi=%.log) $(DVI:%.dvi=%.out) \
  $(DVI:%.dvi=%.bbl) $(DVI:%.dvi=%.blg) $(DVI:%.dvi=%.brf) \
  $(DVI:%.dvi=%.lof) $(DVI:%.dvi=%.lot) $(DVI:%.dvi=%.toc) \
  $(DVI:%.dvi=%.idx) $(DVI:%.dvi=%.ilg) $(DVI:%.dvi=%.ind) \
  $(DVI:%.dvi=%.tid) $(DVI:%.dvi=%.tin) $(DVI:%.dvi=%.tms) \
  $(DVI:%.dvi=%.nlo) $(DVI:%.dvi=%.nls)

cvs :
	cvs ci -m "backup $(shell date -u '+%A, %d %b %Y, %H:%M')"


####################### Info Targets ##############################

warns	: $(SRC)
	  @$(show-warnings)

stats	: $(SRC)
	  @$(show-stats)

show-depend :
	  @echo "# sources   : " $(SRC)
	  @echo "# classes   : " $(CLASSES)
	  @echo "# styles    : " $(STYLES)
	  @echo "# inputs    : " $(INPUTS)
	  @echo "# biblios   : " $(BIBFILE)
	  @echo "# bibstyles : " $(BIBSTYLES)
	  @echo "# encodings : " $(INPUTENCS)
	  @echo "# images    : " $(EPSPICS)

depend :
	  @rm -f Makefile.bak*
	  @csplit Makefile -s -f Makefile.bak "/^\# BEGIN DEPENDENCIES/2" "/^\# END DEPENDENCIES/-1"
	  @rm -f Makefile.bak01
	  @echo > Makefile.bak01
	  @echo "SRC       := $(SRC)      "  > Makefile.bak01
	  @echo "CLASSES   := $(CLASSES)  " >> Makefile.bak01
	  @echo "STYLES    := $(STYLES)   " >> Makefile.bak01
	  @echo "INPUTS    := $(INPUTS)   " >> Makefile.bak01
	  @echo "BIBFILE   := $(BIBFILE)  " >> Makefile.bak01
	  @echo "BIBSTYLES := $(BIBSTYLES)" >> Makefile.bak01
	  @echo "INPUTENCS := $(INPUTENCS)" >> Makefile.bak01
	  @echo "EPSPICS   := $(EPSPICS)  " >> Makefile.bak01
	  @cat Makefile.bak00 Makefile.bak01 Makefile.bak02 > Makefile.bak
	  @rm -f Makefile.bak0*
	  @mv Makefile.bak Makefile
	  @make show-depend


###################### File generation ############################

$(DVI)	: %.dvi : %.tex $(INPUTS) $(DEP) $(BIBFILE) $(INPUTENCS) $(EPSPICS) $(CLASSES) $(STYLES) $(BIBSTYLES)
	@$(run-complete)
	@$(show-warnings)
	@echo ; true
	@$(show-stats)

$(PSF)	: %.ps : %.dvi
	@sed -e "s/[[]dvipdfm[]]/[dvips]/g" $(<:%.dvi=%.tex) > $(<:%.dvi=%.tex.bak)
	@$(rerun-latex)
	@$(DVIPS) $< -o $@

$(PDF)  : %.pdf : %.dvi
	@sed -e "s/[[]dvips[]]/[dvipdfm]/g" $(<:%.dvi=%.tex) > $(<:%.dvi=%.tex.bak)
	@$(rerun-latex)
	@$(DVIPDF) -o $@ $<

$(HTML)	:	%.html : %.tex $(DEP)
	@$(TTH) $<

$(HTM)	:	%_htm : %.tex $(DEP) $(BIBFILE)
	mkdir -p $@
	@$(L2H) -dir $@ $(SRC)
	touch -r $< $@

$(TARNAME) : $(SRC) $(DVI:%.dvi=%.bbl) $(DVI:%.dvi=%.pdf) $(CLASSES) $(STYLES) $(INPUTS) $(BIBFILE) $(BIBSTYLES) $(INPUTENCS) $(EPSPICS) Makefile figs/*.[^e][^p][^s]
	tar -C.. -c -v -z --exclude=CVS -f $@ $(foreach file,$^,$(DIRNAME)/$(file)) > /dev/null


==> ch20.tex <==

% ==============================================================
% Pontificia Universidade Catolica do Rio de Janeiro
% D.Sc. Thesis
%
% Thesis: The Pythagorean Theorem
% Author: Pythagoras of Samos
% Advisor: Thales of Miletus
%
% A Famous Theorem
% ==============================================================



% --------------------------------------------------------------
\chapter{Quaternions}
\label{chapter20}


 --------------------------------------------------------------

%Quaternions%

%Escrever a interpretacao dos quaternios visto como matrizes. Fazer isso tambem para as aplicacoes de recobrimento, escrever as aplicacoes como %





%definicao de aplicacao de \emph{recobrimento} tanto em S3 quanto em S3XS3%



We are identify $\mathbb{R}^{4}$ with the quaternion algebra $\mathbbm{H}$ and $\S^{3}$ with the group of unit quaternions.
It is well-known that $\S^{3} \times \S^{3}$ is the universal double cover of $SO(4)$. The homomorphism $\Pi: \S^{3} \times \S^{3} \rightarrow SO(4)$ which maps any $(\omega_{l},\omega_{r})$ in $\S^{3} \times \S^{3}$ to the isometry $\Pi_{\omega_l,\omega_r}$ defined by 
\begin{equation}\label{rec4}
\Pi_{\omega_l,\omega_r}(z) = \omega_{l} \cdot z \cdot {\omega_{r}}^{-1}, \quad z \in \mathbb{H}
\end{equation}
is surjective, with kernel $\mathbb{Z}_{2}= \lbrace\mathbbm{\pm(1,1)} \rbrace$ and $\Pi$ is a map covering, that gives $\S^{3} \times \S^{3}$ as a 2-sheeted cover of $SO(4)$. 


Identify $\mathbb{R}^{3}$ with the subspace of $\mathbb{H}$ 
generated by the pure imaginary quaternions. We also can restrict $\Pi$ to elements of the diagonal  $\S^{3}=\{(\omega,\omega)\}\subset \S^{3} \times \S^{3}$ and then get the universal double cover  $\Pi:\S^{3} \rightarrow SO(3)$, $u \mapsto \omega \cdot u \cdot \omega^{-1}.$ \label{rec3}
Note that $\Pi_{\omega,\omega}$ is a orthogonal linear transformation of $\mathbb{R}^{4}$ such that $\Pi_{\omega,\omega}(\mathbbm{1})=\mathbbm{1}$. Therefore the subspace $\{0\} \times \mathbb{R}^{3}$ consisting of  pure imaginary quaternions is invariant under $\Pi_{\omega,\omega}$. Thus $\Pi_{\omega,\omega}(u)$ belongs to $SO(3)$.

Let $Q \in SO(4)$, $\Pi^{-1}(Q)=\pm(z_l,z_r)\in \S^{3} \times \S^{3}$ and $\gamma \in {\mathcal{L}\S^{3}}(Q) \subset {\mathcal{I}\S^{3}}(Q)$. The curve $\mathcal{F_{\gamma}}:[0,1] \rightarrow SO(4)$ can be lifted to a unique curve $\tilde{\mathcal{F}}_{\gamma}:[0,1] \rightarrow \S^{3} \times \S^{3}$ such that $\tilde{\mathcal{F}}_{\gamma}(0)=(\mathbbm{1,1})$ and $\Pi \circ \tilde{\mathcal{F}_{\gamma}} = \mathcal{F}_\gamma$. The value of $\tilde{\mathcal{F}}_{\gamma}(1)$ define two spaces 
${\mathcal{L}\S^{3}}((z_l,z_r))$ and 
${\mathcal{L}\S^{3}}((-z_l,-z_r))$ such that 
${\mathcal{L}\S^{3}}(Q)={\mathcal{L}\S^{3}}((z_l,z_r)) \sqcup {\mathcal{L}\S^{3}}((-z_l,-z_r))$. So, ${\mathcal{L}\S^{3}}((z_l,z_r))$ is the space of locally convex curves in $\S^3$ such that $\tilde{\mathcal{F}}_{\gamma}(0)=(\mathbbm{1,1})$ and $\tilde{\mathcal{F}}_{\gamma}(1)=(z_l,z_r)$.  Analogously, we denote $ {\mathcal{I}\S^{3}}(z_l,z_r)$ as the space of immersion curves $\gamma$ in $\S^{3}$ such that $\tilde{\mathcal{F}}_{\gamma}(0)=(\mathbbm{1,1})$ and $\tilde{\mathcal{F}}_{\gamma}(1)=(z_l,z_r)$.

On the same way, given $z \in \S^{3}$ we denote by ${\mathcal{L}\S^{2}}(z)$ (respect. $\mathcal{I}\S^{2}(z) $) the space of locally convex (respect. immersion) curves $\gamma$ in $\S^{2}$ such that $\tilde{\mathcal{F}}_{\gamma}(0)=\mathbbm{1}$ and $\tilde{\mathcal{F}}_{\gamma}(1)=z$.
talvez escrever aqui a notacao para Q em So3, analogo ao anterior.



fazer um paragrafo falando sobre os resultados ja obtidos (como no artigo do nicolau e do boris)
falar do nosso objetivo problema citado no artigo do nicolau e do boris




definicao de derivada logaritmica tanto em so3 como em so4

a cara da matriz da derivada logaritmica de uma curva locally convex

depois disso falar da derivada da aplicacao projecao.


Given a curve $\Gamma: [0,1] \rightarrow SO(4)$, we define it's logarithmic derivative as $\Lambda: [0,1] \rightarrow so(4)$ by $\Lambda (t)= (\Gamma(t))^{-1} \cdot \Gamma ^{'}(t) $.
Let's consider $\mathcal{J} \in so(4)$ as the subset of  skew symmetric matrices, tridiagonal with positive subdiagonal entries, ie., $\mathcal{J}$ is the set of skew Jacobian matrices. The elements of $\mathcal{J}$ are like below, where $j_1$, $j_2$, $j_3$ are positives real numbers
\begin{equation} 
\begin{pmatrix}
0 & -j_1 & 0 & 0 \\
j_1 & 0 & -j_2   & 0 \\
0& j_2  & 0 & -j_3 \\
0 & 0 & j_3  & 0

\end{pmatrix}.
\end{equation}

Let $\Gamma: [0,1] \rightarrow SO(4)$, we call $\Gamma$ a \emph{Jacobian curve} if  $\Lambda (t)= (\Gamma(t))^{-1} \cdot \Gamma ^{'}(t)$ belongs to $\mathcal{J}$.

An important result that help as so much was proving by "Nicolau and Boris (colocar bibli)" and tell us that given a smooth curve $\Gamma:I \rightarrow SO(n+1)$, $\Gamma(0)=I$ we have that $\Gamma$ is a Jacobian curve if and only if   
exist a curve $\gamma \in \mathcal{L}S^{n}$ with $\mathcal{F}_{\gamma}(t)=\Gamma(t)$, for all $t \in I$.

entra a definicao de Gammao Tilda holonomica

falar da derivada da aplicacao Pi e que a Derivada da  Gammao Tilda holonomica mora em ...

escrever como conseguir uma curva gaminha local convex atraves de uma Gammao, pegar a primeira coluna

escrever como conseguir explicitamente uma curva gaminha comecanda na identidade e terminando em determinada Q em Bru At.
 
dada uma curva locally convex escrever a cara da derivada logaritimica tanto para n=2 qt para n=3.

condicoes para uma matriz de jacobi ser frame de uma locally convex curve in S3

\begin{equation} \label{logaritimica4}
\Lambda(t)=
\begin{pmatrix}
0 & -|\gamma'(t)| & 0 & 0 \\
|\gamma'(t)| & 0 & -|\gamma'(t)| \cdot \kappa(t) & 0 \\
0&  |\gamma'(t)| \cdot \kappa(t) & 0 & -|\gamma'(t)| \cdot \tau(t)\\
0 & 0 & |\gamma'(t)| \cdot \tau(t)  & 0

\end{pmatrix}.
\end{equation}

\begin{equation} 
\Lambda(t)=
\begin{pmatrix}
0 & -(b_l(t)-b_r(t))& -(c_l(t)-c_r(t)) & -(d_l(t)-d_r(t)) \\
b_l(t)-b_r(t) & 0 & -(d_l(t)+d_r(t)) &  -(-c_l(t)-c_r(t)) \\
c_l(t)-c_r(t)& d_l(t)+d_r(t)  & 0 & -(b_l(t)+b_r(t))\\
d_l(t)-d_r(t) & -c_l(t)-c_r(t) & b_l(t)+b_r(t)  & 0

\end{pmatrix}.
\end{equation}


\begin{equation} \label{logaritimica_lr}
\Lambda(t)=
\begin{pmatrix}
0 & -(b_l(t)-b_r(t))& 0 & 0 \\
b_l(t)-b_r(t) & 0 & -2 \cdot d(t) & 0 \\
0&  2 \cdot d(t) & 0 & -(b_l(t)+b_r(t))\\
0 & 0 & b_l(t)+b_r(t)  & 0

\end{pmatrix}.
\end{equation}

\begin{equation} \label{logaritimica3}
\Lambda(t)=
\begin{pmatrix}
0 & -|\gamma'(t)| & 0  \\
|\gamma'(t)| & 0 & -|\gamma'(t)| \cdot \kappa(t) \\
0&  |\gamma'(t)| \cdot \kappa(t) & 0  

\end{pmatrix}.
\end{equation}

\begin{equation} \label{logaritimica3}
\Lambda(t)=
\begin{pmatrix}
0 & -2 \cdot d(t) & 0  \\
2 \cdot d(t) & 0 & -2 \cdot b(t) \\
0&  2 \cdot b(t) & 0  

\end{pmatrix}.
\end{equation}

\begin{equation}      
\mathbbm{i}_l=
\begin{pmatrix}
0 & -1 & 0 & 0 \\
+1 & 0 & 0 & 0 \\
0& 0 & 0  & -1 \\
0 & 0 & +1 & 0

\end{pmatrix}.
\end{equation}


\begin{equation} 
\mathbbm{j}_l=
\begin{pmatrix}
0 & 0 & -1 & 0 \\
0 & 0 & 0 & +1 \\
+1 & 0 & 0  & 0 \\
0 & -1 & 0 & 0

\end{pmatrix}.
\end{equation}

\begin{equation} 
\mathbbm{k}_l=
\begin{pmatrix}
0 & 0 & 0 & -1 \\
0 & 0 & -1 & 0 \\
0 & +1 & 0  & 0 \\
+1 & 0 & 0 & 0

\end{pmatrix}.
\end{equation}

\begin{equation} 
\mathbbm{i}_r=
\begin{pmatrix}
0 & +1 & 0 & 0 \\
-1 & 0 & 0 & 0 \\
0 & 0 & 0  & -1 \\
0 & 0 & +1 & 0

\end{pmatrix}.
\end{equation}

\begin{equation} 
\mathbbm{j}_r=
\begin{pmatrix}
0 & 0 & +1 & 0 \\
0 & 0 & 0 & +1 \\
-1 & 0 & 0  & 0 \\
0 & -1 & 0 & 0

\end{pmatrix}.
\end{equation}

\begin{equation} 
\mathbbm{k}_r=
\begin{pmatrix}
0 & 0 & 0 & +1 \\
0 & 0 & -1 & 0 \\
0 & +1 & 0  & 0 \\
-1 & 0 & 0 & 0

\end{pmatrix}.
\end{equation}

$\Pi: S^{3} \times S^{3} \rightarrow SO(4)$,
$(a_l \mathbbm{1}+ b_l \mathbbm{i} + c_l \mathbbm{j} + d_l \mathbbm{k}, a_r \mathbbm{1}+ b_r \mathbbm{i} + c_r \mathbbm{j} + d_r \mathbbm{k}) \mapsto (a_l \cdot I + b_l \cdot \mathbbm{i}_l + c_l \cdot \mathbbm{j}_l + d_l \cdot \mathbbm{k}_l) \cdot (a_r \cdot I + b_r \cdot \mathbbm{i}_r + c_r \cdot \mathbbm{j}_r + d_r \cdot \mathbbm{k}_r) =  (a_r \cdot I + b_r \cdot \mathbbm{i}_r + c_r \cdot \mathbbm{j}_r + d_r \cdot \mathbbm{k}_r) \cdot (a_l \cdot I + b_l \cdot \mathbbm{i}_l + c_l \cdot \mathbbm{j}_l + d_l \cdot \mathbbm{k}_l)$


==> ch88.tex <==

% ==============================================================
% Pontificia Universidade Catolica do Rio de Janeiro
% D.Sc. Thesis
%
% Thesis: The Pythagorean Theorem
% Author: Pythagoras of Samos
% Advisor: Thales of Miletus
%
% A Famous Theorem
% ==============================================================



% --------------------------------------------------------------
\chapter{Characterization of convexity in $\mathcal{L}\SS^3(-\1,\k)$ and $\mathcal{L}\SS^3(\1,-\1)$}

\label{chapter8}



In this section, we give the proof of Theorem~\ref{th2} and Theorem~\ref{th3} that characterizes convexity in the spaces $\mathcal{L}\SS^3(-\1,\k)$ and $\mathcal{L}\SS^3(\1,-\k)$, by just looking at the left part of the curves.

\section{Proof of Theorem~\ref{th2}}\label{s81}


\begin{proof}[{} of Theorem~\ref{th2}]
Recall that we want to prove that a curve $\gamma \in \mathcal{L}\SS^3(-\1,\k)$ is convex if and only its left part $\gamma_l \in \mathcal{L}\SS^2(-\1)$ is convex.

It is clear that $\mathcal{L}\SS^2(-\1)$ contains convex curves; the curve $\sigma_c$, for $0 < c <2\pi$ defined in~\S\ref{s72} is convex, since it intersects any hyperplane of $\R^3$ (or equivalently any great circle) in exactly two points. Using Theorem~\ref{thmani}, the space $\mathcal{L}\SS^2(-\mathbf{1})$ has therefore $2$ connected components,
\[ \mathcal{L}\SS^2(-\mathbf{1})=\mathcal{L}\SS^2(-\mathbf{1})_c \sqcup \mathcal{L}\SS^2(-\mathbf{1})_n \]
where $\mathcal{L}\SS^2(\mathbf{1})_c$ is the component associated to convex curves and $\mathcal{L}\SS^2(\mathbf{1})_n$ the component associated to non-convex curves.

The space $\mathcal{L}\SS^3(-\1,\k)$ also contains convex curves. Indeed, recall the family of curves $\gamma_{1}^m \in \mathcal{L}\SS^3((-\1)^m,\k^m)$, $m \geq 1$, defined in Example~\ref{family1}; we will prove that the curve $\gamma_{1}^1 \in \mathcal{L}\SS^3(-\1,\k)$ is convex. Up to a reparametrization with constant speed, this curve is the same as the curve $\tilde{\gamma} : [0,\pi/2] \rightarrow \SS^3$ defined by
\begin{eqnarray*}
\tilde{\gamma}(t) & = & \left(\frac{1}{4}\cos\left(3t\right)+\frac{3}{4}\cos\left(t\right)\right., \\
&  & \frac{\sqrt{3}}{4}\sin\left(3t \right)+\frac{\sqrt{3}}{4}\sin\left(t\right) \\
&  & \frac{\sqrt{3}}{4}\cos\left(t\right)-\frac{\sqrt{3}}{4}\cos\left(3t\right) \\
&  & \left.\frac{3}{4}\sin\left(t\right)-\frac{1}{4}\sin\left(3t \right)\right).
\end{eqnarray*} 
Since being convex is independent of the choice of a parametrization (Chapter~\ref{chapter3}, \S\ref{s32}, $(i)$ of Proposition~\ref{propconv}), it is sufficient to prove that $\tilde{\gamma}$ is convex. Observe that for $t \in [0,\pi/2)$, the first component of $\tilde{\gamma}$ never vanishes, so if we define the central projection
\[ p : (x_1,x_2,x_3,x_4) \in \R^4 \mapsto \left(1,\frac{x_2}{x_1},\frac{x_3}{x_1},\frac{x_4}{x_1}\right), \]
then it is sufficient to prove that the curve $p(\tilde{\gamma})$, defined for $t \in [0,\pi/2)$: this follows from $(ii)$ of Corollary~\ref{corconv}, Chapter~\ref{chapter3}, \S\ref{s32}. We compute
\[ p(\tilde{\gamma}(t))=\left(1,\sqrt{3}\tan t,\sqrt{3}(\tan t)^2,(\tan t)^3\right) \]
and hence, if we reparametrize by setting $x=\tan t$, we obtain the curve
\[ x \in [0,+\infty) \mapsto (1,\sqrt{3}x,\sqrt{3}x^2,x^3) \in \R^4. \]
It is now obvious that this curve is convex, and therefore our initial curve $\gamma_1^1$ is convex. As before, using Theorem~\ref{thmani}, the space $\mathcal{L}\SS^3(-\mathbf{1},\k)$ has therefore $2$ connected components,
\[ \mathcal{L}\SS^3(-\mathbf{1},\k)=\mathcal{L}\SS^3(-\mathbf{1},\k)_c \sqcup \mathcal{L}\SS^3(-\mathbf{1},\k)_n \]
where $\mathcal{L}\SS^3(\mathbf{1},\k)_c$ is the component associated to convex curves and $\mathcal{L}\SS^3(\mathbf{1},\k)_n$ the component associated to non-convex curves.

Then we can use Theorem~\ref{th1} to define a continuous map
\[ L : \mathcal{L}\SS^3(-\mathbf{1},\k) \rightarrow \mathcal{L}\SS^2(-\mathbf{1})  \]
by setting $L(\gamma)=\gamma_l$, where $(\gamma_l,\gamma_r)$ is the pair of curve associated to $\gamma$. . Since $L$ is continuous and $\mathcal{L}\SS^3(-\mathbf{1},\k)_c$, its image by $L$ is also connected. Moreover, we know $\gamma_1^1 \in \mathcal{L}\SS^3(-\mathbf{1},\k)_c$, and that $L(\gamma_1^1)=\sigma_1 \in \mathcal{L}\SS^2(-\mathbf{1})_c$, therefore the image of $\mathcal{L}\SS^3(-\mathbf{1},\k)_c$ by $L$ intersects $\mathcal{L}\SS^2(-\mathbf{1})_c$; since the latter is connected we must have the inclusion
\[ L\left(\mathcal{L}\SS^3(-\mathbf{1},\k)_c\right) \subset \mathcal{L}\SS^2(-\mathbf{1})_c. \]
This proves one part of the statement, namely that if $\gamma \in \mathcal{L}\SS^3(-\mathbf{1},\k)_c$, then its left part $\gamma_l=L(\gamma) \in \mathcal{L}\SS^2(-\mathbf{1})_c$. To prove the other part, it is enough to prove that    
\[ L\left(\mathcal{L}\SS^3(-\mathbf{1},\k)_n\right) \subset \mathcal{L}\SS^2(-\mathbf{1})_n. \]
To prove this inclusion, using continuity and connectedness arguments as before, it is enough to find one element in $\mathcal{L}\SS^3(-\mathbf{1},\k)_n$ whose image by $L$ belongs to $\mathcal{L}\SS^2(-\mathbf{1})_n$. We claim that the curve $\gamma_1^5$ from Example~\ref{family1} do the job. To see that $\gamma_1^5 \in \mathcal{L}\SS^3(-\mathbf{1},\k)$, one easily check that if we define the plane 
\[ H=\{(x_1,0,0,x_4) \in \R^4 \; | \; x_1 \in \R, \; x_4 \in \R\} \]  
then
\[ \gamma_5(t_i) \in H, \quad t_i=\frac{i}{5}, \quad 1 \leq i \leq 4. \]
Hence $\gamma_5$ has at least $4$ points of intersection with $H$; this shows that $\gamma_5$ is not convex. To conclude, it is clear that $L(\gamma_5)=\sigma_5 \in \mathcal{L}\SS^2(-\mathbf{1})_n$. Hence this proves the inclusion we wanted, and this concludes the proof.

\end{proof}  

\section{Proof of Theorem~\ref{th3}}\label{s82}


